Engaging with AI: How Interface Design Shapes Human-AI Collaboration in High-Stakes Decision-Making

As reliance on AI systems for decision-making grows, it becomes critical to ensure that human users can appropriately balance trust in AI suggestions with their own judgment, especially in high-stakes domains like healthcare. However, human + AI teams have been shown to perform worse than AI alone, with evidence indicating automation bias as the reason for poorer performance, particularly because humans tend to follow AI's recommendations even when they are incorrect. In many existing human + AI systems, decision-making support is typically provided in the form of text explanations (XAI) to help users understand the AI's reasoning. Since human decision-making often relies on System 1 thinking, users may ignore or insufficiently engage with the explanations, leading to poor decision-making. Previous research suggests that there is a need for new approaches that encourage users to engage with the explanations and one proposed method is the use of cognitive forcing functions (CFFs). In this work, we examine how various decision-support mechanisms impact user engagement, trust, and human-AI collaborative task performance in a diabetes management decision-making scenario. In a controlled experiment with 108 participants, we evaluated the effects of six decision-support mechanisms split into two categories of explanations (text, visual) and four CFFs. Our findings reveal that mechanisms like AI confidence levels, text explanations, and performance visualizations enhanced human-AI collaborative task performance, and improved trust when AI reasoning clues were provided. Mechanisms like human feedback and AI-driven questions encouraged deeper reflection but often reduced task performance by increasing cognitive effort, which in turn affected trust. Simple mechanisms like visual explanations had little effect on trust, highlighting the importance of striking a balance in CFF and XAI design.

==> main/related_work.tex <==
\section{Related Work}\label{related_work}
%please be sure to include prior work from HCI here that has already development several projects related to making meal choices, maybe for weight loss or other reasons, but the fundamental concern of using a machine to help you make a decision has been explored and our work builds on that with generative AI giving us the ability to now tell the user why the machine made a specific decision to help improve trust.

==> main/theory.tex <==
\section{Theory and Framework}

We will first introduce the theoretical foundation of our work, and then present the framework we use to evaluate the effectiveness of decision support mechanisms in influencing user trust, engagement and decision-making in an AI-based system. 
Given the critical role that trust plays in human-AI interaction, particularly in high-stakes decision-making, our framework is grounded in the theories of trust in AI system and cognitive load.

\subsection{Theoretical Foundations}
\subsubsection{Trust in AI Systems}

Trust in human-AI interaction is a complex and multifaceted construct that influences user behavior and decision-making. It emphasizes the dynamic nature of trust, which evolves based on the system's performance and user experiences~\cite{}. 
Misaligned trust can lead to suboptimal decision-making. Overtrust may result in users blindly following AI suggestions without sufficient scrutiny, while undertrust may cause users to dismiss valuable AI insights~\cite{}.
Existing research emphasizes the importance of transparency and explainability in building human trust in AI systems~\cite{}. However, recent studies suggest that while these factors are necessary, they may be not sufficient to prevent overreliance on AI~\cite{}. Cognitive load theory suggests that if the cognitive effort required to understand AI outputs is too high, users may choose for trust out of convenience, rather than engaging critically with the AI's suggestions~\cite{}. 

\subsubsection{Cognitive Load and User Engagement}

Cognitive load theory provides a manner to understand how the mental effort to process information affects user engagement and decision-making. The theory differentiates between intrinsic load (task complexity), extraneous load (how information is presented), and germane load (the cognitive effort required to process and integrate information). 
In human-AI interaction, cognitive load is relevant when users are presented with AI explanations or confidence levels. If the information is overwhelming or too complex, users may experience cognitive overload, leading them to accept AI suggestions without critical evaluation. On the other hand, if the information is too simplistic, users may not trust the AI's suggestions~\cite{}. 




\subsection{Framework}
Based on the theoretical foundations, we propose a framework to guild the evaluation of AI support mechanisms. Our framework integrates trust calibration, cognitive load management, and human-AI collaboration to understand how different AI interactions influence user behavior. 

\subsubsection{Hypotheses}
\begin{enumerate}
    \item H1: Visual explanations provide intuitive and easily interpretable information and will reduce extraneous cognitive load. Thus encourage users to either trust or critically evaluate AI outputs.
    \item H2: Detailed textual explanations will enhance trust by increasing transparency and perceived integrity of the AI's decision-making process.
    \item H3: Confidence levels serve as a quantifiable metric that provides users with direct insight into the AI's certainty. This will help users to calibrate their trust in the AI system.
    \item H4: Allowing users to input confidence levels will encourage users to compare their judgment with the AI's, forcing them to critically evaluate the AI's suggestions.
    \item H5: AI-driven questions will promote users to reflect on AI outputs and encourage deeper  cognitive processing and critical evaluation.
    \item H6: Behavior visualization will help users evaluate the AI's reliability and consistency over time, adjusting their trust levels based on empirical evidence rather than initial impressions.
\end{enumerate}



\subsubsection{Evaluation Metrics}
Our evaluation metrics include: ...
